The Spectrometer Development of CosmoCube, Lunar Orbiting Satellite to Detect 21-cm Hydrogen Signal from Cosmic Dark Ages

The cosmic Dark Ages represent a pivotal epoch in the evolution of the Universe, marked by the emergence of the first cosmic structures under the influence of dark matter. The 21-cm hydrogen line, emanating from the hyperfine transition of neutral hydrogen, serves as a critical probe into this era. We describe the development and implementation of the spectrometer for CosmoCube, a novel lunar orbiting CubeSat designed to detect the redshifted 21-cm signal within the redshift range of 13 to 150. Our instrumentation utilizes a Xilinx RFSoC, which integrates both Analog-to-Digital Converters (ADCs) and Digital-to-Analog Converters (DACs), tailored for the spectrometer component of the radiometer. This system is characterized by a 4096 FFT length at 62.5 kHz steps using a Polyphase Filter Bank (PFB), achieving an average Effective Number of Bits (ENOB) of 11.5 bits throughout the frequency of interest, from 10 MHz to 100 MHz. The spectrometer design is further refined through loopback tests involving both DAC and ADC of the RFSoC, with DAC outputs varying between high (+1 dBm) and low (-3 dBm) power modes to characterize system performance. The power consumption was optimized to 5.45 W using three ADCs and one DAC for the radiometer. Additionally, the stability of the ADC noise floor was investigated in a thermal chamber with environmental temperatures ranging from 5{\deg}C to 40{\deg}C. A consistent noise floor of approximately -152.5 dBFS/Hz was measured, with a variation of $\pm$0.2 dB, ensuring robust performance under varying thermal conditions.

==> IDEAS.tex <==


The modeled absorption feature, generated using an Emulator of the Dark Ages 21-cm signal built with GLOBAEMU \citep{Bevins2021} and approximated with the RECFAST code \citep{Acharya2022}, shows varying depths depending on the baryon density and the reduced Hubble constant. As either the baryon density or the reduced Hubble constant increases, the 21-cm signal's absorption feature during the Dark Ages deepens.

\textbf{As \cite{Anstey2021} demonstrates the modeled absorption feature of 21-cm signal in Dark Ages via GLOBAEMU \citep{Bevins2021}, shows varying depths depending on the baryon density ($\Omega_b$) and the reduced Hubble constant ($h$). The research showing either $\Omega_b$ or h increases, the 21-cm signal's absorption feature during the Dark Ages deepens. In a $\Lambda\text{CDM}$ universe, the signal strength aligned with Planck's measurement of $h$ \citep{Planck2018} is about 10 mK shallower compared to that inferred from the SH0ES measurement \citep{Riess_2022}. Hence, we aim to achieve 10 mK sensitivity through the passive and active components used in the front end, as well as the calibration. }

\begin{comment}
\textbf{The reasoning behind 6.6 being considered 99.9\% Gaussian noise peak to peak is discussed in another application note by Analog Devices \href{https://www.analog.com/media/en/technical-documentation/application-notes/an-615.pdf}{this link}.}
\end{comment}

\textbf{Details on Why NAD RSS and Pfund RMS in Analog Devices' tutorial \href{https://www.analog.com/media/en/training-seminars/tutorials/MT-003.pdf}{this link}.}

ENOB calculation 
\text{https://scdn.rohde-schwarz.com/ur/pws/dl_downloads/dl_application/application_notes/1er03/ENOB_Technical_Paper_1ER03_1e.pdf}

Why NAD RSS and Pfund RMS.
https://www.analog.com/media/en/training-seminars/tutorials/MT-003.pdf#:~:text=Six%20popular%20specifications%20for%20quantifying,(spurious%20free%20dynamic%20range).

https://www.analog.com/media/en/technical-documentation/application-notes/an-615.pdf why 6.6 is 99.9\% gaussian noise peak to peak.

Noise 6.6
https://www.renesas.com/us/en/document/ppt/understanding-noise-signal-chain

enob
https://www.xilinx.com/content/dam/xilinx/support/documents/white_papers/wp509-rfsampling-data-converters.pdf

THEPAPER CHECK FOR BRAM UTILIZATION
https://iopscience.iop.org/article/10.1088/1748-0221/16/08/P08047/pdf


\begin{figure}
    \centering
    % Adjust the trim values as needed: trim={<left> <lower> <right> <upper>}
    \includegraphics[width=\columnwidth,trim=1.2cm 6.3cm 2.5cm 7.1cm, clip]{PolyPhaseFilterBank.pdf}
    \caption{PFB Solid line with 8 ntaps and 140 stop band attenuation. Dashed 4 ntaps and 140 stop band attenuation. Dotted 4 ntaps and 100 stop band attenuation.}
    \label{fig:your_label}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\columnwidth, trim=14.45cm 20.92cm 9.08cm 0.92cm, clip]{CosmuCubeStructure.pdf}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw[-{Latex[length=1mm,width=1mm]}] (0.74,0.74) -- (0.74,0.68) node[near start, above, yshift=1mm, align=left] {Deployed Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.68,0.25) -- (0.62,0.25) node[near start, right, xshift=1.5mm, align=left] {Solar Panels};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.57) -- (0.38,0.57) node[near start, left, xshift=-1mm, align=left] {Stowed Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.5) -- (0.38,0.5) node[near start, left, xshift=-1mm, align=left] {Electronic Stack};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.39) -- (0.38,0.39) node[near start, left, xshift=-1mm] {Battery};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.3) -- (0.38,0.3) node[near start, left, xshift=-1mm, align=left] {CosmoCube Controller};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.21) -- (0.38,0.21) node[near start, left, xshift=-1mm, align=left] {Communication Box};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.1) -- (0.38,0.16) node[near start, left, xshift=-1mm, align=left] {Patch Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.68,0.1) -- (0.62,0.1) node[near start, right, xshift=1.5mm, align=left] {Thrusters};
        \end{scope}
    \end{tikzpicture}
    \caption{CosmoCube with annotation (size of each instrument not to scale)}
    \label{fig:cosmocube_annotated}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\columnwidth, trim=8cm 6cm 9.08cm 0.92cm, clip]{StowedCosmoCube.pdf}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw[-{Latex[length=1mm,width=1mm]}] (0.74,0.74) -- (0.74,0.68) node[near start, above, yshift=1mm, align=left] {Deployed Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.68,0.25) -- (0.62,0.25) node[near start, right, xshift=1.5mm, align=left] {Solar Panels};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.57) -- (0.38,0.57) node[near start, left, xshift=-1mm, align=left] {Stowed Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.5) -- (0.38,0.5) node[near start, left, xshift=-1mm, align=left] {Electronic Stack};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.39) -- (0.38,0.39) node[near start, left, xshift=-1mm] {Battery};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.3) -- (0.38,0.3) node[near start, left, xshift=-1mm, align=left] {CosmoCube Controller};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.21) -- (0.38,0.21) node[near start, left, xshift=-1mm, align=left] {Communication Box};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.34,0.1) -- (0.38,0.16) node[near start, left, xshift=-1mm, align=left] {Patch Antenna};
            \draw[-{Latex[length=1mm,width=1mm]}] (0.68,0.1) -- (0.62,0.1) node[near start, right, xshift=1.5mm, align=left] {Thrusters};
        \end{scope}
    \end{tikzpicture}
    \caption{CosmoCube with annotation (size of each instrument not to scale)}
    \label{fig:cosmocube_annotated}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\columnwidth, trim=0cm 8cm 0cm 11cm, clip]{CosmuCubeStructureLRGantenna.pdf}};
    \end{tikzpicture}
    \caption{CosmoCube with annotation (size of each instrument not to scale)}
    \label{fig:cosmocube_annotated}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\columnwidth, trim=0cm 12cm 0cm 6cm, clip]{CosmuCubeStructureLRGantenna2.pdf}};
    \end{tikzpicture}
    \caption{CosmoCube with annotation (size of each instrument not to scale)}
    \label{fig:cosmocube_annotated}
\end{figure}
